HEAT: Holistic Edge Attention Transformer for Structured Reconstruction

This paper presents a novel attention-based neural network for structured reconstruction, which takes a 2D raster image as an input and reconstructs a planar graph depicting an underlying geometric structure. The approach detects corners and classifies edge candidates between corners in an end-to-end manner. Our contribution is a holistic edge classification architecture, which 1) initializes the feature of an edge candidate by a trigonometric positional encoding of its end-points; 2) fuses image feature to each edge candidate by deformable attention; 3) employs two weight-sharing Transformer decoders to learn holistic structural patterns over the graph edge candidates; and 4) is trained with a masked learning strategy. The corner detector is a variant of the edge classification architecture, adapted to operate on pixels as corner candidates. We conduct experiments on two structured reconstruction tasks: outdoor building architecture and indoor floorplan planar graph reconstruction. Extensive qualitative and quantitative evaluations demonstrate the superiority of our approach over the state of the art. Code and pre-trained models are available at https://heat-structured-reconstruction.github.io.

==> texts/figures/filtering_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/filtering_example.pdf}
    \caption{A toy example to illustrate the candidate filtering.\ym{Do we really need such a figure???} }
    \label{fig:filtering}
\end{figure}

==> texts/tables/table_hawp_results.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{HAWP baseline
    }
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 5pt
	    \begin{tabu}{@{\;} cccc @{\quad\;\;} ccccccccc@{\;}}
	        \addlinespace
	        \toprule
	        {Data Type} & \multicolumn{9}{c}{ Outdoor Satellite Images}  \\ 
	        {Eval Type} & & \multicolumn{3}{c}{Corner} &  \multicolumn{3}{c}{Edge} &  \multicolumn{3}{c}{Region} \\
	        Image size & Train epochs & Prec & Recall & F-1 & Prec & Recall & F-1 & Prec & Recall & F-1  \\
	        \midrule
	        256  & 30*4 & 80.4 & 84.7 & 82.5 & 61.9 & 71.7 & 66.4 & 49.4 & 59.6 & 54.0  \\
	        256 & 100*4 & 85.6 & 82.9 & 84.2 & 73.3 & 68.6 & 70.9 & 69.2 & 58.6 & 63.4 \\
	        256 & 200*4 & 89.6 & 82.4 & 85.8 & 76.6 & 68.1 & 72.1 & 74.1 & 55.4 & 63.4 \\
	        512 & 30*4 & 81.2 & 87.9 & 84.4 & 65.5 & 77.9 & 71.2 & 61.2 & 66.5 & 63.7 \\
	        512 & 100*4 & 85.7 & 86.7 & 86.2 & 76.7 & 73.9 & 75.2 & 74.0 & 59.6 & 66.0 \\
	        512 & 200*4 & 89.1 & 84.6 & 86.8 & 78.8 & 72.0 & 75.2 & 77.5 & 57.8 & 66.2 \\
    	    \bottomrule
	    \end{tabu}
	}
    \label{tab:hawp}
\end{table*}

==> texts/tables/table_letr_results.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{LETR baseline
    }
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 5pt
	    \begin{tabu}{@{\;} ccccc @{\quad\;\;} ccccccccc@{\;}}
	        \addlinespace
	        \toprule
	        {Data Type} & \multicolumn{9}{c}{ Outdoor Satellite Images}  \\ 
	        {Eval Type} & & & \multicolumn{3}{c}{Corner} &  \multicolumn{3}{c}{Edge} &  \multicolumn{3}{c}{Region} \\
	        Image size & Query num & Stage num & Prec & Recall & F-1 & Prec & Recall & F-1 & Prec & Recall & F-1  \\
	        \midrule
	        256 & 50 & 1 & 81.5 & 73.3 & 77.1 & 55.7 & 53.3. & 54.4 & 65.1 & 38.5 & 48.4    \\
	        256 & 50 & 2 & 85.9 & 74.9 & 80.0 & 59.1 & 58.3 & 58.7 & 67.2 & 45.2 & 54.0 \\
	        256 & 50 & 3 &  85.8 & 74.7 & 79.8 & 58.4 & 57.9 & 58.2 & 66.8 & 45.1 & 53.8 \\
	        \midrule
	        256 & 100 & 1 & 84.5 & 73.4 & 78.5 & 57.8 & 54.9 & 56.3 & 66.1 & 42.6 & 51.8 \\
	        256 & 100 & 2 & 87.7 & 74.7 & 80.7 & 60.4 & 58.9 & 59.7 & 67.4 & 48.2 & 56.2 \\
	        256 & 100 & 3 & 87.8 & 74.8 & 80.8 & 59.7 & 58.6 & 59.1 & 68.3 & 48.7 & 56.8  \\
	        \midrule
	        256 & 150 & 1 & 84.5 & 71.7 & 77.5 & 55.2 & 52.1 & 53.6 & 59.5 & 39.7 & 47.6 \\
	        256 & 150 & 2 & 87,7 & 74.0 & 80.3 & 59.1 & 57.6 & 58.4 & 61.3 & 44.8 & 51.8 \\
	        256 & 150 & 3 & 87.9 & 74.0 & 80.4 & 59.0 & 57.9 & 58.4 & 61.8 & 44.9 & 52.0 \\
	        \midrule
	        256 & 200 & 1 & 81.9 & 74.6 & 78.1 & 58.1 & 55.2 & 56.6 & 67.9 & 38.3 & 49.0 \\
	        256 & 200 & 2 & 85.0 & 75.7 & 80.1 & 59.8 & 59.6 & 59.7 & 69.4 & 44.7 & 54.4 \\
	        256 & 200 & 3 & 85.1 & 75.9 & 80.3 & 60.0 & 60.1 & 60.1 & 70.9 & 46.2 & 56.0  \\
	        \midrule
	        256 & 400 & 1 & \multicolumn{3}{l}{Not converged}  \\
	        \midrule
	        512 & 100 & 1 & 89.6 & 79.1 & 84.0 & 64.2 & 66.6 & 65.4 & 73.7 & 55.7 & 63.4  \\
	        512 & 100 & 2 & 90.5 & 79.5 & 84.7 & 64.1 & 68.6 & 66.3 & 74.3 & 59.8 & 66.3 \\
	        512 & 100 & 3 & 90.1 & 79.1 & 84.2 & 62.6 & 68.3 & 65.3 & 73.2 & 60.2 & 66.1 \\
	        \midrule
	        512 & 200 & 1 & 90.7 & 79.5 & 84.7 & 66.3 & 69.4 & 67.8 & 76.8 & 58.6 & 66.4  \\
	        512 & 200 & 2 & 90.7 & 79.6 & 84.8 & 65.4 & 71.5 & 68.3 & 77.5 & 63.1 & 69.6 \\
	        512 & 200 & 3 & 90.3 & 79.7 & 84.7 & 64.0 & 71.6 & 67.6 & 77.1 & 62.6 & 69.1 \\
    	    \bottomrule
	    \end{tabu}
	}
    \label{tab:letr}
\end{table*}
